Hierarchical prosody modeling and control in non-autoregressive parallel neural TTS

Neural text-to-speech (TTS) synthesis can generate speech that is indistinguishable from natural speech. However, the synthetic speech often represents the average prosodic style of the database instead of having more versatile prosodic variation. Moreover, many models lack the ability to control the output prosody, which does not allow for different styles for the same text input. In this work, we train a non-autoregressive parallel neural TTS front-end model hierarchically conditioned on both coarse and fine-grained acoustic speech features to learn a latent prosody space with intuitive and meaningful dimensions. Experiments show that a non-autoregressive TTS model hierarchically conditioned on utterance-wise pitch, pitch range, duration, energy, and spectral tilt can effectively control each prosodic dimension, generate a wide variety of speaking styles, and provide word-wise emphasis control, while maintaining equal or better quality to the baseline model.

==> content/prosody.tex <==

% Read more, references from Parallel Tacotron and CHiVE papers \cite{wan2019chive}

Traditionally, prosody modeling is based on schematizing and labeling prosodic phenomena and developing rule-based systems or statistical models from the derived data \cite{Prosody2010}. However, the prosodic attributes are difficult and time-consuming to annotate, and therefore such an approach is impractical for modern TTS with large databases. In contrast, end-to-end neural TTS systems learn prosody as an inherent part of the model, which makes the generation of speech with the correct linguistic content and the appropriate prosody a consistent modeling task. However, such prosodically unsupervised models lack the explicit control over the output prosody.

Recent developments in end-to-end neural TTS have provided some solutions to prosody modeling. In \cite{skerryryan2018endtoend}, an extension to the Tacotron architecture is introduced to capture the residual attributes that are not specified by the linguistic input. The model learns a latent embedding space of prosody through conditional auto-encoding, derived from the target Mel-spectrograms, to enable prosody transfer.

As an improvement to \cite{skerryryan2018endtoend}, \cite{Wang2018StyleTU} proposed global style tokens (GSTs) to learn a clustered latent space of prosody. The same prosody encoder as in \cite{skerryryan2018endtoend} is used, but a style token layer is added where the prosody embedding is used as a query to an attention layer that maps the embedding to the GSTs using combination weights. The output of the style token layer is a style embedding that describes the prosodic style. The architecture can be used for either prosody transfer using a reference audio or for directly generating a specific prosodic style by choosing a style token.

The aforementioned unsupervised methods for learning a latent space of prosody have many advantages. Unsupervised methods do not need any extra information or labeling of prosody, and all the components are jointly trained to achieve a consistent model. However, there are some drawbacks. First, the latent space represents all the residual acoustic differences in the reference Mel-spectrograms after linguistic content has been accounted for. As a result, any acoustic differences due to channel (recording setup, noise type and level) and (undesirable) variability in speaker's voice from one day to another are also learned. Therefore, instead of focusing on meaningful prosodic aspects of speech, the model learns an entangled representation of prosody and unknown underlying acoustic factors. Second, manual listening of the tokens is required to determine what sort of style tokens the model has learned from the data, and how to utilize these for reproducing a desired prosody. Third, the number of style tokens must be set heuristically, and the model is not guaranteed to find perceptually distinct and prosodically meaningful clusters for each of the tokens. The individual style tokens are often either similar to each other, or it may be hard to make practical use of the learned style tokens as they may not represent any desired styles.

The prosody of language covers all aspects of speech that are not related directly to the articulation for the linguistic expression. Although there is no agreed number of prosodic variables, there is a set of variables that is widely agreed to have a major contribution to prosody. These variables are 1) pitch, 2) length of the speech sounds, 3) loudness, and 4) timbre or voice quality \cite{Campbell2003vq,Sluijter1996SpectralBA}. These four subjective auditory variables can be accurately measured using the following acoustic variables: fundamental frequency, phone duration, speech energy, and spectral tilt, respectively. Assuming that the four acoustic features cover the prosodic space, then there are certain benefits in using them for prosody modeling and control: 1) they are disentangled so that they can be independently varied, 2) they are intuitive so that it is easy to understand their effect on prosody, 3) they are independent from other acoustic factors, such as background noise or other recordings conditions, thus making them robust for prosody modeling.

In this work, we will directly utilize the four dimensions of prosody, described by the corresponding acoustic features, hierarchically both in a coarse-grained and fine-grained form, to model and control the prosody of synthetic speech.
